OSWorld: Benchmarking Multimodal Agents for Open-Ended Tasks in Real Computer Environments

Autonomous agents that accomplish complex computer tasks with minimal human interventions have the potential to transform human-computer interaction, significantly enhancing accessibility and productivity. However, existing benchmarks either lack an interactive environment or are limited to environments specific to certain applications or domains, failing to reflect the diverse and complex nature of real-world computer use, thereby limiting the scope of tasks and agent scalability. To address this issue, we introduce OSWorld, the first-of-its-kind scalable, real computer environment for multimodal agents, supporting task setup, execution-based evaluation, and interactive learning across various operating systems such as Ubuntu, Windows, and macOS. OSWorld can serve as a unified, integrated computer environment for assessing open-ended computer tasks that involve arbitrary applications. Building upon OSWorld, we create a benchmark of 369 computer tasks involving real web and desktop apps in open domains, OS file I/O, and workflows spanning multiple applications. Each task example is derived from real-world computer use cases and includes a detailed initial state setup configuration and a custom execution-based evaluation script for reliable, reproducible evaluation. Extensive evaluation of state-of-the-art LLM/VLM-based agents on OSWorld reveals significant deficiencies in their ability to serve as computer assistants. While humans can accomplish over 72.36% of the tasks, the best model achieves only 12.24% success, primarily struggling with GUI grounding and operational knowledge. Comprehensive analysis using OSWorld provides valuable insights for developing multimodal generalist agents that were not possible with previous benchmarks. Our code, environment, baseline models, and data are publicly available at https://os-world.github.io.

==> text/tables/comparison.tex <==
% \begin{table*}[htbp]
% \centering
% \caption{
% \tao{a bit too long}\sz{agree, some benchmarks are less relevant anyway (e.g., scienceworld, virtualhome, alfred), maybe simply mention them in related work is enough.} \sz{Maybe consider redesign this table to \emph{highlight} the key features of \ours.}
% Comparison of \ours to other exisiting digital agent benchmarks.
% We provide an executable environment that unifies the observation spaces of CLI and GUI, supporting various operating systems and a universal action space for agents to learn and evaluate. 
% We offer a variety of setups for Initial States to simulate real-world scenarios for agents and use the ratio of evaluation scripts to the number of examples to reflect task diversity and evaluation reliability.
% \tao{REAL cross os (open-ended tasks, desktop apps, focus on environment instead of just benchmark -), cross-applications, interfaces - not just obs? nl tasks? different ways showing eval, initial... no -oriented/... obs space -> exe. environment, digital universal -> keyword \& mouse, intermediate env start setup scripts - explore context, eval, }
% % \tao{to add visualwebarena/WebLINX}
% \tianbao{Define and demonstrate the \#eval scripts/\#examples; Demonstrate the #environments in different aspects; Open-ended task type. Add AssistGUI, OmniACT (all task udner the current single screenshot; executable environment, 1, evaluation semantic matching; 2, exclude possible solution); mention POMDP as a aspect}
% % \tao{
% % 1) "Doc provided" is weak, think about more unique dimensions, e.g., showing 
% % a.) 1 desktop env covers more than web/app/coding/bash... much larger env space and action space..... 
% % b.) reliable exe-based eval, 
% % c.) cross-app task examples,... 
% % d.) macos, windows, ubuntu? 
% % d) different initial states 
% % 2) move it to page 2 or 3. 
% % 3) confusing symbols in task resources, 
% % 4) also include agentbench and gaia - not just web/mobile... our work as general agent env including coding/bash.... 
% % 5) env initial setup? more unique points? 
% % 6) can have better column names
% % }
% }
% \label{tab:comparison-benchmarks}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \thead{Benchmark} & \thead{\footnotesize Exec.\\ \footnotesize Env.?}  &\thead{Obs.\\ Space} & \thead{Act.\\ Space} & \thead{Avg.\\ Steps} & \thead{\#Initial States} & \thead{\footnotesize \#Eval. Scripts \\/ \footnotesize \#Examples} \\ 
% \midrule
% \textsc{\footnotesize Form/QAWoB}~\citep{shi2017world}  & {\textcolor{red}{\ding{55}}} & Web Page & Web-Oriented 
% & - & - & - \\
% \textsc{\footnotesize MiniWoB++}~\citep{liu2018reinforcement} & {\textcolor{green}{\ding{51}}} & Web Page & Web-Oriented 
% & 2.3 & 128 & 128/128 \\
% \textsc{\footnotesize MineDojo}~\citep{fan2022minedojo} & {\textcolor{green}{\ding{51}}} &  Game & Game-Specific 
% & - & 74   & 4/1581 \\
% \textsc{\footnotesize WebShop}~\citep{yao2022webshop} & {\textcolor{green}{\ding{51}}} &  Web Page & Web-Oriented 
% & 11.3 & 1  & 1/500  \\
% \textsc{\footnotesize WikiHow}~\citep{zhang2023mobile} & \textcolor{green}{\ding{51}} & Mobile & Tap-Based \includegraphics[width=0.3cm,height=0.3cm]{images/logos/tap.png}  
% & 5.6 & 1 & 14/150 \\
% \textsc{\footnotesize SheetCopilot}~\cite{li2023sheetcopilot} & {\textcolor{red}{\ding{55}}} & tbd & tbd
% & tbd & tbd  & tbd \\
% \textsc{\footnotesize Mind2Web}~\citep{deng2023mind2web} & {\textcolor{red}{\ding{55}}} &  Web Page & Web-Oriented
% & 7.3 & - & - \\
% \textsc{\footnotesize InterCode}~\citep{yang2023intercode} & {\textcolor{green}{\ding{51}}} &  Bash/SQL/Python & Code-Only 
% & - & 1/1/1 & - \\
% \textsc{\footnotesize WebArena}~\citep{zhou2023webarena} & {\textcolor{green}{\ding{51}}} &  Web Page(s) & Web-Oriented 
% & - & 46 & 3/811 \\
% \textsc{\footnotesize AitW}~\cite{rawles2023android} & {\textcolor{red}{\ding{55}}} & Mobile & Tap-Based \includegraphics[width=0.3cm,height=0.3cm]{images/logos/tap.png} 
% & 6.5 & -  & -  \\
% \textsc{\footnotesize AgentBench}~\cite{liu2023agentbench} & {\textcolor{green}{\ding{51}}} & Database/Game/... & SQL/Game-Specific... 
% & - & -  & 8/1141 \\
% \textsc{\footnotesize GAIA}~\cite{mialon2023gaia} & {\textcolor{red}{\ding{55}}} & N/A & N/A 
% & - & -  & 1/466 \\
% \textsc{\footnotesize AgentBoard}~\cite{ma2024agentboard} & {\textcolor{red}{\ding{55}}} & tbd & tbd
% & tbd & tbd  & tbd \\
% \textsc{\footnotesize VWebArena}~\cite{Koh2024VisualWebArenaEM} & {\textcolor{red}{\ding{55}}} & tbd & tbd
% & tbd & tbd  & tbd \\
% \textsc{\footnotesize WebLINX}~\cite{lu2024weblinx} & {\textcolor{red}{\ding{55}}} & tbd & tbd
% & tbd & tbd  & tbd \\

% \midrule
% \thead{\footnotesize \ours \footnotesize (Ours)} & {\textcolor{green}{\ding{51}}} & \thead{Operating System \\ \footnotesize Ubuntu, Windows, macOS, \textit{etc}} & \thead{Digital Universal\\ \includegraphics[width=0.3cm,height=0.3cm]{images/logos/cursor.png} \includegraphics[width=0.4cm,height=0.3cm]{images/logos/keyboard.png}} 
% & 12.9 & 130 & \numevals/\numexamples \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


\begin{table*}[htbp]
\centering
\caption{
}
\label{tab:comparison-benchmarks}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\thead{Benchmark} & \thead{\footnotesize Exec.\\ \footnotesize Env.?}  &\thead{Obs.\\ Space} & \thead{Act.\\ Space} & \thead{Avg.\\ Steps} & \thead{\#Initial States} & \thead{\footnotesize \#Eval. Scripts \\/ \footnotesize \#Examples} \\ 
\midrule
\textsc{\footnotesize Form/QAWoB}~\citep{shi2017world}  & {\textcolor{red}{\ding{55}}} & Web Page & Web-Oriented 
& - & - & - \\
\textsc{\footnotesize MiniWoB++}~\citep{liu2018reinforcement} & {\textcolor{green}{\ding{51}}} & Web Page & Web-Oriented 
& 2.3 & 128 & 128/128 \\
\textsc{\footnotesize MineDojo}~\citep{fan2022minedojo} & {\textcolor{green}{\ding{51}}} &  Game & Game-Specific 
& - & 74   & 4/1581 \\
\textsc{\footnotesize WebShop}~\citep{yao2022webshop} & {\textcolor{green}{\ding{51}}} &  Web Page & Web-Oriented 
& 11.3 & 1  & 1/500  \\
\textsc{\footnotesize WikiHow}~\citep{zhang2023mobile} & \textcolor{green}{\ding{51}} & Mobile & Tap-Based \includegraphics[width=0.3cm,height=0.3cm]{images/logos/tap.png}  
& 5.6 & 1 & 14/150 \\
\textsc{\footnotesize SheetCopilot}~\cite{li2023sheetcopilot} & {\textcolor{red}{\ding{55}}} & tbd & tbd
& tbd & tbd  & tbd \\
\textsc{\footnotesize Mind2Web}~\citep{deng2023mind2web} & {\textcolor{red}{\ding{55}}} &  Web Page & Web-Oriented
& 7.3 & - & - \\
\textsc{\footnotesize InterCode}~\citep{yang2023intercode} & {\textcolor{green}{\ding{51}}} &  Bash/SQL/Python & Code-Only 
& - & 1/1/1 & - \\
\textsc{\footnotesize WebArena}~\citep{zhou2023webarena} & {\textcolor{green}{\ding{51}}} &  Web Page(s) & Web-Oriented 
& - & 46 & 3/811 \\
\textsc{\footnotesize AitW}~\cite{rawles2023android} & {\textcolor{red}{\ding{55}}} & Mobile & Tap-Based \includegraphics[width=0.3cm,height=0.3cm]{images/logos/tap.png} 
& 6.5 & -  & -  \\
\textsc{\footnotesize AgentBench}~\cite{liu2023agentbench} & {\textcolor{green}{\ding{51}}} & Database/Game/... & SQL/Game-Specific... 
& - & -  & 8/1141 \\
\textsc{\footnotesize GAIA}~\cite{mialon2023gaia} & {\textcolor{red}{\ding{55}}} & N/A & N/A 
& - & -  & 1/466 \\
\textsc{\footnotesize AgentBoard}~\cite{ma2024agentboard} & {\textcolor{red}{\ding{55}}} & tbd & tbd
& tbd & tbd  & tbd \\
\textsc{\footnotesize VWebArena}~\cite{Koh2024VisualWebArenaEM} & {\textcolor{red}{\ding{55}}} & tbd & tbd
& tbd & tbd  & tbd \\
\textsc{\footnotesize WebLINX}~\cite{lu2024weblinx} & {\textcolor{red}{\ding{55}}} & tbd & tbd
& tbd & tbd  & tbd \\

\midrule
\thead{\footnotesize \ours \footnotesize (Ours)} & {\textcolor{green}{\ding{51}}} & \thead{Operating System \\ \footnotesize Ubuntu, Windows, macOS, \textit{etc}} & \thead{Digital Universal\\ \includegraphics[width=0.3cm,height=0.3cm]{images/logos/cursor.png} \includegraphics[width=0.4cm,height=0.3cm]{images/logos/keyboard.png}} 
& 12.9 & 130 & \numevals/\numexamples \\
\bottomrule
\end{tabular}
}
\end{table*}

